Near-linear time approximation algorithms for optimal transport via Sinkhorn iteration

Computing optimal transport distances such as the earth mover's distance is a fundamental problem in machine learning, statistics, and computer vision. Despite the recent introduction of several algorithms with good empirical performance, it is unknown whether general optimal transport distances can be approximated in near-linear time. This paper demonstrates that this ambitious goal is in fact achieved by Cuturi's Sinkhorn Distances. This result relies on a new analysis of Sinkhorn iteration, which also directly suggests a new greedy coordinate descent algorithm, Greenkhorn, with the same theoretical guarantees. Numerical simulations illustrate that Greenkhorn significantly outperforms the classical Sinkhorn algorithm in practice.

==> commands.tex <==

\usepackage{amsmath, amssymb, color}
\usepackage{amsthm} 
%\usepackage{natbib}
\usepackage[colorlinks,citecolor=blue,urlcolor=blue]{hyperref}
\usepackage{xcolor,colortbl}
%
\RequirePackage{hypernat}
\usepackage{cleveref}
%
\usepackage{color}
\usepackage{amsfonts, fancybox}
\usepackage{amssymb}
\usepackage[american]{babel}
% \addto{\captionsamerican}{\renewcommand{\abstractname}{}}
%
\usepackage{psfrag,color}
\usepackage{dcolumn}
% \usepackage{subfigure}
\usepackage[format=hang, justification=justified, singlelinecheck=false]{subcaption}
\usepackage{flafter, bm, dsfont}
\usepackage[section]{placeins}
\usepackage[final]{showkeys}
\renewcommand*\showkeyslabelformat[1]{%
\fbox{\normalfont\tiny\ttfamily#1}}


\usepackage{multirow}
\usepackage{color}
\usepackage{amsmath}
\usepackage{float}
\usepackage{mathrsfs}
\usepackage{amsfonts}
\usepackage{dsfont}
\usepackage{amssymb}
%
%\usepackage{algorithmic, algorithm}
\usepackage{wrapfig}
\usepackage[overload]{textcase}


\usepackage{amssymb, latexsym}

%
\usepackage{graphicx}
%
\usepackage{epstopdf}
\usepackage{tikz}
\usepackage{pgfplots}
\usepgfplotslibrary{fillbetween}

%% if you need to pass options to natbib, use, e.g.:
%% \PassOptionsToPackage{numbers, compress}{natbib}
%% before loading nips_2017
%%
%% to avoid loading the natbib package, add option nonatbib:
%%\usepackage[nonatbib]{nips_2017}
%
%%\usepackage[nonatbib]{nips_2017}
%
%% to compile a camera-ready version, replace the above line with the following, which has the [final] option, e.g.:
%% \usepackage[final]{nips_2017}
%
%\usepackage[utf8]{inputenc} % allow utf-8 input
%\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
%\usepackage{hyperref}       % hyperlinks
%\usepackage{url}            % simple URL typesetting
%\usepackage{booktabs}       % professional-quality tables
%\usepackage{amsfonts}       % blackboard math symbols
%\usepackage{nicefrac}       % compact symbols for 1/2, etc.
%\usepackage{microtype}      % microtypography
%\usepackage{wrapfig}        % for wrapping figures
%\usepackage[notref, notcite, final]{showkeys}
%
%\usepackage{amsmath, amsthm, amsfonts}
%\usepackage{dsfont}
%\usepackage[sort]{cite}
%\usepackage{graphicx}
%
%% Notes
\usepackage{color}
\newcommand{\jw}[1]{{\textcolor{red}{[\textbf{JON:} #1]}}}
%\newcommand{\pr}[1]{{\textcolor{blue}{[\textbf{PR:} #1]}}}
%
%% For algorithms
\usepackage{algorithm}
%%\usepackage[noend]{algorithmic}
\usepackage[noend]{algcompatible}
%
%% Theorem definitions
\newtheorem{defin}{Definition}%[section]
\newtheorem{thm}{Theorem}%[section]
\newtheorem{exe}{Exercise}%[section]
\newtheorem{exa}{Example}%[section]
\newtheorem{fact}{Fact}%[section]
\newtheorem{prop}{Proposition}%[section]
\newtheorem{lemma}{Lemma}%[section]
\newtheorem{corol}{Corollary}%[thm]
\newtheorem{conj}{Conjecture}%[section]
\newtheorem{remark}{Remark}%[section]
\newtheorem{discussion}{Discussion}%[section]
\newtheorem{conc}{Conclusion}%[section]

% Custom definitions

\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}

\newcommand{\bA}{\mathbf{A}}
\newcommand{\bB}{\mathbf{B}}
\newcommand{\bC}{\mathbf{C}}
\newcommand{\bD}{\mathbf{D}}
\newcommand{\bE}{\mathbf{E}}
\newcommand{\bF}{\mathbf{F}}
\newcommand{\bG}{\mathbf{G}}
\newcommand{\bH}{\mathbf{H}}
\newcommand{\bI}{\mathbf{I}}
\newcommand{\bJ}{\mathbf{J}}
\newcommand{\bK}{\mathbf{K}}
\newcommand{\bM}{\mathbf{M}}
\newcommand{\bN}{\mathbf{N}}
\newcommand{\bO}{\mathbf{O}}
\newcommand{\bP}{\mathbf{P}}
\newcommand{\bQ}{\mathbf{Q}}
\newcommand{\bS}{\mathbf{S}}
\newcommand{\bT}{\mathbf{T}}
\newcommand{\bU}{\mathbf{U}}
\newcommand{\bV}{\mathbf{V}}
\newcommand{\bX}{\mathbf{X}}
\newcommand{\bY}{\mathbf{Y}}
\newcommand{\bZ}{\mathbf{Z}}


%\renewcommand{\subseteq}{\subset}

\newcommand{\R}{{\rm I}\kern-0.18em{\rm R}}
\newcommand{\h}{{\rm I}\kern-0.18em{\rm H}}
\newcommand{\PP}{{\rm I}\kern-0.18em{\rm P}}
\newcommand{\E}{{\rm I}\kern-0.18em{\rm E}}
\newcommand{\Z}{{\rm Z}\kern-0.18em{\rm Z}}
\newcommand{\1}{{\rm 1}\kern-0.24em{\rm I}}
\newcommand{\N}{{\rm I}\kern-0.18em{\rm N}}

\newcommand{\DS}{\displaystyle}
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmin}{argmin}
\newcommand{\Tr}{\mathrm{Tr}}
\newcommand{\eps}{\varepsilon}
\newcommand{\del}{\delta}
\newcommand{\re}{\R}
\newcommand{\calN}{\mathcal{N}}
\newcommand{\plusminus}{\raisebox{.2ex}{$\scriptstyle\pm$}}
\newcommand{\nnz}{\text{nnz}}
%\DeclareMathOperator*{\KL}{D_{\mathrm{KL}}}
\newcommand{\KL}{\cK}
\newcommand{\half}{\frac{1}{2}}
\newcommand{\diag}{\mathbf{D}}
\newcommand{\ones}{\bone_n}
\newcommand{\tildo}{\widetilde{O}}
\newcommand{\rbar}{\bar{r}}
\newcommand{\cbar}{\bar{c}}
\newcommand{\bone}{\mathbf{1}}
\newcommand{\0}{\mathbf{0}}

\newcommand{\errr}{\text{err}_r}
\newcommand{\errrp}{\text{err}_r^{(+)}}
\newcommand{\errrn}{\text{err}_r^{(-)}}
\newcommand{\errc}{\text{err}_c}
\newcommand{\errcp}{\text{err}_c^{(+)}}
\newcommand{\errcn}{\text{err}_c^{(-)}}
\newcommand{\Cinfty}{\|C\|_{\infty}}

\newcommand{\zeroesr}{\text{zeroes}_r}
\newcommand{\zeroesc}{\text{zeroes}_c}

\newcommand{\Pavg}{P_{\text{avg}}}
\newcommand{\Pavgex}{P_{\text{avg}}^{\text{exact}}}
\newcommand{\Ptex}{P_t^{\text{exact}}}
\newcommand{\Pbar}{{\bar{P}}}
\newcommand{\Pprime}{P'}
\newcommand{\Pex}{Q^{\text{sink}}}
\newcommand{\Qsink}{\Pex}
\newcommand{\Poptprime}{(P^*)'}

\newcommand{\U}{\cU_{r,c}}
\newcommand{\Ubar}{\cU_{\rbar, \cbar}}
\newcommand{\Uprime}{\cU_{r', c'}}
\newcommand{\dist}{\mathrm{dist}}
\newcommand{\Peta}{P_\eta}
\newcommand{\sink}{\Pi_{\cS}}

% algorithm names (feel free to change these!)
\newcommand{\lmdot}{\textsc{lmdot}}
\newcommand{\ot}{\textsc{ApproxOT}}
\newcommand{\lmd}{\textsc{lmd}}
\newcommand{\roundtrans}{\textsc{round}}
\newcommand{\approxsink}{\textsc{approxsinkhorn}}
\newcommand{\sinkhorn}{\textsc{Sinkhorn}}
\newcommand{\threshold}[1]{\textsc{threshold}_{#1}}
\newcommand{\approxproj}{\textsc{Proj}}
\newcommand{\greedy}{\textsc{Greenkhorn}}
